Data-Augmented and Retrieval-Augmented Context Enrichment in Chinese Media Bias Detection

With the increasing pursuit of objective reports, automatically understanding media bias has drawn more attention in recent research. However, most of the previous work examines media bias from Western ideology, such as the left and right in the political spectrum, which is not applicable to Chinese outlets. Based on the previous lexical bias and informational bias structure, we refine it from the Chinese perspective and go one step further to craft data with 7 fine-grained labels. To be specific, we first construct a dataset with Chinese news reports about COVID-19 which is annotated by our newly designed system, and then conduct substantial experiments on it to detect media bias. However, the scale of the annotated data is not enough for the latest deep-learning technology, and the cost of human annotation in media bias, which needs a lot of professional knowledge, is too expensive. Thus, we explore some context enrichment methods to automatically improve these problems. In Data-Augmented Context Enrichment (DACE), we enlarge the training data; while in Retrieval-Augmented Context Enrichment (RACE), we improve information retrieval methods to select valuable information and integrate it into our models to better understand bias. Extensive experiments are conducted on both our dataset and an English dataset BASIL. Our results show that both methods outperform our baselines, while the RACE methods are more efficient and have more potential.

==> figures/fig_eda_anno_features.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{pictures/eda_ps.pdf}
    % \includegraphics[width=0.42\textwidth]{pictures/eda_ps.eps}
    \caption{
   Training results with EDA perturbing labeled words.
   $x$-axis: varying proportion labeled words replaced/deleted by EDA.
  $y$-axis: F1 difference compared to the original all-policy EDA with random selection.
    %The influence of annotation features in all policies augmentation. The leftmost result shows the experiment with all labeled tokens are kept. The farther to the right, the higher proportion of labelled words in replacement and deletion operations.
    }
    \label{fig:eda_p}
    % \vspace{-.4cm}
\end{figure}

==> latex_files/6result.tex <==
% \section{Context Enrichment Results}
% \input{tables/combined_results}


% \subsection{Results of DACE}
% % \subsection{Data-Augmented Enrichment}

% % The EDA and UDA methods enrich the phrases and sentences in the training, we can regard them as corpus enrichment methods.
% In DACE, SR, RI, RS, RD, and EDA are supervised learning methods with augmentation in the token level, while UDA is a semi-supervised learning method that augments the data in the sentence level.

% \newparagraph{Token-Level Enrichment}
% From \Cref{tb:combined_result}, we observe that the policies of EDA in general enable BERT to perform better, although there are minor differences among each policy, indicating the overall helpfulness of data augmentation on our task.
% All four types of policies help to increase the scale of the training set, while the policy RI enriches the word corpus without content reduction, which shows better performance than other policies.
% % Compared with the policies SR and RD, RI shows better performance.

% In conclusion, implementing the four policies together increases the robustness of the performance, and gained improvements in all tasks.
% This further confirms that EDA is suitable to be used as a noise-adding approach in UDA, which can maintain the consistency of label distribution in media bias detection tasks.






% \newparagraph{Sentence-Level Enrichment}
% From \Cref{tb:combined_result}, we observe that UDA method further enhances the performance of media bias detection, especially in lexical bias detection.
% To further explore how UDA functions, we conduct experiments in several steps with the increase in the percentage of unlabeled sentences feeding to the model, and the results of each task are shown in \Cref{fig:uda_n}.

% As the scale of training sentences increases, the performance of Coarse-Grained Combined grows continuously with small fluctuations. While the situations are quite different in Fine-Grained classification tasks.
% The F1 score of the Fine-Grained lexical bias task first rapidly drops then increases slowly, and maintains an upward trend.
% While there is a lot of fluctuation in the curve of the Fine-Grained informational bias task.
% The results indicate that enrichment in training corpus has a significant effect on lexical bias detection however the improvements in informational bias are unstable, which is also aligned with their natural features.

% When go through the details of the predictions in the model, we observe the UDA's improvements in overfitting. 
% It is more sensitive about the biased sentence and can better distinguish the trigger words.
% For example, most of the sentences with \textit{Opinion} have the token ''believe'', while the word can also be used for other purposes. UDA can avoid labeling all the sentences with ''believe'' as biased sentences.
% Our experiments also verify that large-scale of unlabeled data can be used to enlarge the training set of some practical tasks with small-scale datasets and get improvements in the performance. Also, semi-supervised and even unsupervised learning has the potential to be further explored in the future.


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{pictures/uda_n1.pdf}
%     \caption{Results of UDA with different scales of unlabeled data.
%    $x$-axis: varying percentage of the extended dataset as unlabeled sentences when training UDA.
%   $y$-axis: F1 score.}
%     \label{fig:uda_n}
% \end{figure}





% \subsection{Results of RACE}

% \label{sec:irmethods}


% \newparagraph{Information Retrieval}
% Our RACE results are also shown in \Cref{tb:combined_result}.
% From our ground truth model BERT+Context, adding external context sentences improves the results, which is aligned with the result of previous work \cite{van2020context}.
% Some information retrieval methods are conducted to select valuable information from external knowledge source.
% We can observe that the gap between traditional and neural network methods is not as large as other tasks. But the traditional method BM25 is weak in informational bias detection, deep learning models can make up and have more potential in this field.
% SimCSE and DPR have similar performance in informational bias performance. While the SimCSE model outperforms other models in lexical bias detection, because we fine-tune the SimCSE model based on a large pre-training language model, which already contains a lot of semantic information.


% \newparagraph{Combining Titles}
% When the titles are also added as the context of the sentence, from \Cref{tb:combined_result}, we notice that DPR+title gets best performance in general. Compared with the model only consider the single sentence itself, the combination of titles helps to retrieval more precise and valuable information.
% While the way to feeding titles is also important, concatenating the title and the sentence simply even sometimes hurts the performances.
% DPR model is more flexible, which can encode the titles and sentences separately, takes full advantage of the titles and further improves the results.

% We also notice the shortage of our model in considering time series. For example, there is a case that the target sentence is, 

% \textit{``If the authorities still further restrict demonstrations and gatherings, they may have exceeded public health safety considerations."} 

% We find the context sentences through model DPR+title, for example,

% \textit{``Egypt opened the Rafah port connecting the Gaza Strip on the same day, allowing hundreds of Palestinians stranded in Egypt due to the epidemic to return to Palestine"}, 

% \textit{``From May 16th to 19th, the ``stay-at-home order" will continue to be implemented nationwide"}, 

% \textit{``The spread of the epidemic in India is accelerating"}.

% These sentences are similar to the target sentence in semantics, and can also provide information on epidemic situations of other countries as references. However, they will also bring confusion if the description is not for the same period.
% The original design of DPR is for the QA system, most of the queries and answers are about general knowledge which seldom changes as time goes on.   
% While one of the significant differences between our task and the QA task is that reports in journalism are time-sensitive, which indicates us the future direction of improvement in the models.








% \subsection{Case Study}
% % We observe that the data augmentation methods work better than informational retrieval methods.
% % When analyzing the cases, we have several findings. 

% % One of the significant observations is that UDA performs better in fine-grained classification tasks.

% The adding of retrieved information provides more knowledge and improves the performance is easy to understand. In this part, to provide more insights into what can be learned by UDA, we conduct a case study on fine-grained lexical bias detection to explore the difference between basic BERT and UDA when detecting the bias after a larger scale of training data is supplied. 

% Because there is attention mechanism in both methods, we use the visualization tool BertViz \cite{vig2019multiscale} to show the attention relationship in each layer and head among the tokens.
% When we highlight the words according to the attention matrix, we can find that the basic BERT can also learn the pattern related to media bias in general, only minor difference appears in UDA, which improves the final performances.


% \Cref{fig:casestudy} shows the attention mechanism of the sentence "Hong Kong people who are in the UK are crazy for the air tickets to avoid quarantine". The ground truth shows that this sentence has lexical bias \textit{Exaggeration}.
% Both of the methods correctly classify the bias at coarse-grained level, while in fine-grained, basic BERT wrongly classifies it as \textit{Opinion}.
% From \Cref{fig:casestudy}, we obverse that the allocation of attention in basic BERT is more average than that in UDA.
% As we know, in our dataset, informational bias is longer than lexical bias, and \textit{Opinion} is usually longer than other bias in lexical bias.
% Due to the divergence in length of different bias types, it is easier for the model to give the result according to the length of the highlighted part, that is why BERT labels it as \textit{Opinion}.
% We notice that in the result of model UDA, the token ''crazy'', which is the trigger of bias \textit{Exaggeration} in human judgment, got much more attention than other tokens.
% So, when the model cannot exactly find the important tokens may result in an incorrect result in fine-grained level, and UDA, which enrich data-augmented context and make up the gap.




% \begin{figure}[!t]
%     \centering 
%     \subfigure[BERT]{  
%     \begin{minipage}{0.22\textwidth}
%         \centering    
%         \includegraphics[scale=0.62]{pictures/cs1.png}
%     \end{minipage}}
%     \subfigure[UDA]{
%     \begin{minipage}{0.22\textwidth}
%         \centering    
%         \includegraphics[scale=0.62]{pictures/cs2.png}
%     \end{minipage}}
%     \caption{The attention relationship presentation of model BERT and UDA. The darker color stands for larger value in attention parameters.}  
%     \label{fig:casestudy}
% \end{figure}



==> latex_files/7future.tex <==
% \section{ChatGPT and Future Work}
% Recently, ChatGPT, a strong model that interacts in a conversational way, was released by OpenAI. 
% It performs well in almost every task that machines have attempted to do in human current expectations.
% We also use ChatGPT to test our task to find its strengths and weaknesses, so that we can better plan our future work and cooperate with those strong large language models. The results are shown in \Cref{tb:gpt_test}.

% \begin{table}
% \centering
% \small
% \resizebox{0.45\textwidth}{!}{
% \begin{tabular}{c|c|c|c}
% \toprule
% \textbf{Task} & \textbf{HL} ($\downarrow$) & \textbf{JI} ($\uparrow$) & \textbf{F1} ($\uparrow$) \\
% \midrule
% Coarse-Grained & 0.315 & 0.040 & 0.078 \\
% \midrule\midrule
% \textbf{Sub-Task} & \textbf{P} ($\uparrow$) & \textbf{R}($\uparrow$) & \textbf{F1} ($\uparrow$) \\
% \midrule
% Lexical & 0.846 & 0.065 & 0.122 \\
% Informational & 0.400 & 0.014 & 0.026 \\

% \bottomrule
% \end{tabular}
% }
% \caption{The results of bias detection tasks in ChatGPT with zero-shot setting. The experiments are conducted in our dataset with a Coarse-Grained detecting task and its sub-tasks, lexical bias detection, and informational bias detection. We use the same notations as in \Cref{tb:combined_result}}
% \label{tb:gpt_test}
% \end{table}




% \newparagraph{Additional Context}
% From \Cref{tb:gpt_test}, we notice that there is a big difference in the performance of ChatGPT between lexical bias detection and informational bias detection. It is harder for ChatGPT to tell informational bias.
% When a single sentence or a single article is given, ChatGPT usually requests more information before giving the answer, such as the source of the report, or the context of related news.
% Similar to our experiment setting, ChatGPT also needs comparison with other contexts to detect the bias.
% Although much longer contexts are allowed in ChatGPT than in our model, it also has some flaws in understanding the long text, for example, the model sometimes will omit some information when the text is too long.
% However, the limitation in length also exists, we cannot simply input all the contexts we have.
% The retrieval methods are still quite important for searching for valuable information from large knowledge sources as the assistance of bias detection.




% \newparagraph{Fine-grained Bias Detection}
% We can also observe that ChatGPT has high precision but low recall scores.
% As a strong language model, ChatGPT is good at some basic language tasks, such as translation and summarization. The former can bridge the language barrier by translating non-English text into English, and the latter helps to draft a summary, which is a necessary step for informational bias detection and inspires us to apply it to our model in the future.

% Even so, some ironic phrases or sentences are easily misunderstood due to the lack of background culture.
% For example, the original article criticizes that some groups have taken all the achievements, while ChatGPT understands it as a positive tone that praises these groups and results in a misjudgment.
% Also, because the judgment is based on the result of summarization, ChatGPT works better when detecting the bias at the article level.
% Although most of the results and analysis are reasonable, it would not specify the sentence or phrase that the bias is in.
% The bias would be ignored unless we give phrases directly. For example, we tested "Wuhan Virus", which would be ignored within a sentence, but ChatGPT clearly points out that this phrase is not suitable to be used after WTO suggested the formal name of this virus, COVID-19. 
% The above deficiencies result in a low recall score, while our work, which is in fine-grained detection, can much more clearly remind authors or readers to notice potential bias.



==> tables/case_study.tex <==

\begin{table*}[h!]
\centering
\small
\begin{tabular}{p{0.97\textwidth}}
\toprule
\textbf{Writing Bias Prediction Cases}  \\\midrule
They are $[$crazy for$]_\textbf{Exaggeration}$ air tickets, flying around the earth, hoping to "return to $[$the safest$]_\textbf{Exaggeration}$ place". 
\\\midrule
After seeing the outbreak of the epidemic and the British government's $[$"Buddha-like"$]_\textbf{Stereotype / Labelling}$ handling...
\\\midrule
... The actual number of patients is more than announced, and the situation $[$is bound to continue to deteriorate$]_\textbf{Speculative Content / Opinion}$. \\
\bottomrule
\toprule
\textbf{Content Bias Prediction Cases}  \\\midrule
\textbf{\underline{Article 1}}
...$[$He revealed that since the closure of the city, the Taiwan compatriot Ms.Ma and her son Xiaoyu have not stepped out of the house. 
... Under the arrangement of the United Front Work Department and the Affairs Office, a doctor's health certificate diagnosis was carried out, and a blood test and a CT examination were also prepared to bring back together.$]_\textbf{Omission}$
 \\
\midrule
\textbf{\underline{Article 2}}
...The decree mutation raises doubts about the hemophilia patient and his mother's return to Taiwan.
...Airline only stressed that due to personal data issues, the identity of the passengers could not be disclosed.
...$[$However, people familiar with the matter pointed out that concerned departments have arranged a meeting this afternoon to discuss the contingency strategies for them after returning to Taiwan.$]_\textbf{Omission}$
 \\
\midrule
\textbf{\underline{Article 3}}
...The hemophilic teenager was short of medicines because he didn't catch the first flight back to Taiwan.
Delivering medicines across thousands of miles temporarily relieves the problem of insufficient medicines.
$[$Recently, his mother claimed that the life-saving medicine was out again, and he was also in constant trouble due to his nationality issue.$]_\textbf{Error}$
 \\

\bottomrule
\end{tabular}
\caption{case study}
\label{tb:case_study}
\end{table*}


==> tables/eda_result.tex <==
\begin{table*}
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Coarse-Grained}} 
 & \multicolumn{3}{c|}{\textbf{Fine-Grained Combined}} 
 & \multicolumn{3}{c|}{\textbf{Fine-Grained Lexical}}  
 & \multicolumn{3}{c}{\textbf{Fine-Grained Informational}}  \\\cmidrule{2-13}

 & \textbf{HL} ($\downarrow$) & \textbf{JI} ($\uparrow$) & \textbf{F1} ($\uparrow$)
 & \textbf{HL} ($\downarrow$) & \textbf{JI} ($\uparrow$) & \textbf{F1} ($\uparrow$)
 & \textbf{HL} ($\downarrow$) & \textbf{JI} ($\uparrow$) & \textbf{F1} ($\uparrow$)
 & \textbf{HL} ($\downarrow$) & \textbf{JI} ($\uparrow$) & \textbf{F1} ($\uparrow$) \\\midrule
 
  BERT & 0.238 & 0.414 & 0.585 & 
\textbf{0.108} & 0.368 & 0.539 & 
\textbf{0.095} & 0.427 & 0.598 & 
\textbf{0.118} & 0.261 & 0.414 \\\midrule

Synonym Replace & 0.236 & 0.459 & 0.629 & 
0.111 & 0.339 & 0.507 & 
0.097 & 0.411 & 0.583 & 
0.130 & 0.299 & 0.460 \\
 
Random Insertion & \textbf{0.225} & 0.472 & 0.642 & 
\textbf{0.108} & 0.368 & 0.538 & 
0.097 & 0.429 & 0.600 & 
0.138 & \textbf{0.318} & \textbf{0.482}  \\
 
Random Swap & 0.228 & \textbf{0.481} & \textbf{0.649} & 
0.110 & 0.360 & 0.529 & 
0.098 & \textbf{0.433} & \textbf{0.604} & 
0.132 & 0.308 & 0.470  \\
 
Random Deletion & 0.232 & 0.443 & 0.614 & 
0.112 & 0.352 & 0.521 & 
0.100 & 0.414 & 0.585 & 
0.142 & 0.308 & 0.471  \\\midrule

All Policies Above & 0.246 & 0.465 & 0.635 & 
0.116 & \textbf{0.386} & \textbf{0.557} & 
0.100 & 0.423 & 0.594 & 
0.148 & 0.294 & 0.454  \\


 
\bottomrule
\end{tabular}
}
\caption{
Validation results on sentence-level media bias classification with different EDA augmentation policies. 
}
\label{tb:eda}
\end{table*}






==> tables/ir_result.tex <==



\begin{table*}
\centering
\small
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{\textbf{BASIL}} & \multicolumn{6}{c}{\textbf{Our dataset}} \\\cmidrule{2-13}
 & \multicolumn{3}{c|}{\textbf{Lexical}} & \multicolumn{3}{c|}{\textbf{Informational}} & \multicolumn{3}{c|}{\textbf{Lexical}} & \multicolumn{3}{c}{\textbf{Informational}} \\\cmidrule{2-13}
 & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\\midrule
 BERT  & 0.139 & 0.396 & 0.196 & 0.310 & 0.569 & 0.394 & 0.635 & 0.706 & 0.666 & 0.508 & 0.666 & 0.568  \\
 Article Context & \textbf{0.150} & 0.564 & 0.235 & 0.302 & 0.639 & 0.402 & 0.626 & 0.701 & 0.660 & 0.500 & 0.633 & 0.556  \\
 Set Context & 0.143 & 0.572 & 0.227 & \textbf{0.324} & 0.619 & \textbf{0.423} & 0.630 & 0.708 & 0.666 & 0.499 & 0.683 & 0.575  \\\midrule
BM25  & \textbf{0.150} & \textbf{0.671} & \textbf{0.244} & 0.302 & 0.543 & 0.385 & 0.641 & 0.667 & 0.649 & 0.498 & 0.637 & 0.558 \\
SimCSE  & 0.146 & 0.616 & 0.235 & 0.316 & 0.615 & 0.414 & \textbf{0.643} & 0.697 & 0.663 & \textbf{0.515} & 0.685 & \textbf{0.586}  \\
DPR  & 0.139 & 0.588 & 0.223 & 0.315 & 0.621 & 0.415 & 0.631 & \textbf{0.709} & 0.666 & 0.495 & 0.695 & 0.576  
\\\midrule
SimCSE+title  & 0.137 & 0.602 & 0.222 & 0.300 & \textbf{0.642} & 0.404 & 0.633 & 0.708 & 0.666 & 0.496 & 0.687 & 0.574  \\
DPR+title  & 0.147 & 0.635 & 0.239 & 0.319 & 0.616 & 0.419 & 0.639 & \textbf{0.709} & \textbf{0.668} & 0.497 & \textbf{0.708} & 0.583  \\
\bottomrule
\end{tabular}
}
\caption{Results in BASIL and our dataset with several informational retrieval methods. The experiments are conducted separately in lexical and informational bias on the sentence level.
The best performance is marked in bold.}
\label{tb:ir_result}
\end{table*}
